Just Type It in Isabelle! AI Agents Drafting, Mechanizing, and Generalizing from Human Hints

Type annotations are essential when printing terms in a way that preserves their meaning under reparsing and type inference. We study the problem of complete and minimal type annotations for rank-one polymorphic $\lambda$-calculus terms, as used in Isabelle. Building on prior work by Smolka, Blanchette et al., we give a metatheoretical account of the problem, with a full formal specification and proofs, and formalize it in Isabelle/HOL. Our development is a series of experiments featuring human-driven and AI-driven formalization workflows: a human and an LLM-powered AI agent independently produce pen-and-paper proofs, and the AI agent autoformalizes both in Isabelle, with further human-hinted AI interventions refining and generalizing the development.

==> macros.tex <==
% macros.tex
\RequirePackage{xspace}

\newcommand{\smoblacitations}{smo_thesis,smobla_workshop,smobla_journal}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}

% Tools
\newcommand{\toolstyle}[1]{#1\xspace}

% #1 = command name, #2 = display text
\newcommand{\tool}[2]{%
\expandafter\newcommand\csname #1\endcsname{\toolstyle{#2}}%
}

\tool{isabelle}{Isabelle}
\tool{isabellehol}{Isabelle/HOL}
\tool{isabelleml}{Isabelle/ML}
\tool{jedit}{Isabelle/jEdit}
\tool{isar}{Isar}
\tool{sledgehammer}{Sledgehammer}
\tool{iq}{Isabelle/Q}
\tool{opencode}{OpenCode}
\tool{claude}{Claude Opus}

% Dollar sign for costs
\newcommand{\cost}[1]{\$#1}
